Bispectral Neural Networks

We present a neural network architecture, Bispectral Neural Networks (BNNs) for learning representations that are invariant to the actions of compact commutative groups on the space over which a signal is defined. The model incorporates the ansatz of the bispectrum, an analytically defined group invariant that is complete -- that is, it preserves all signal structure while removing only the variation due to group actions. Here, we demonstrate that BNNs are able to simultaneously learn groups, their irreducible representations, and corresponding equivariant and complete-invariant maps purely from the symmetries implicit in data. Further, we demonstrate that the completeness property endows these networks with strong invariance-based adversarial robustness. This work establishes Bispectral Neural Networks as a powerful computational primitive for robust invariant representation learning

==> Bispectral Neural Networks ICLR Camera Ready/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> Bispectral Neural Networks ICLR Camera Ready/sections/0-abstract.tex <==
We present a neural network architecture, Bispectral Neural Networks (BNNs) for learning representations that are invariant to the actions of compact commutative groups on the space over which a signal is defined. The model incorporates the ansatz of the bispectrum, an analytically defined group invariant that is \textit{complete}\textemdash that is, it preserves all signal structure while removing only the variation due to group actions. Here, we demonstrate that BNNs are able to simultaneously learn groups, their irreducible representations, and corresponding equivariant and complete-invariant maps purely from the symmetries implicit in data.  Further, we demonstrate that the completeness property endows these networks with strong invariance-based adversarial robustness. This work establishes Bispectral Neural Networks as a powerful computational primitive for robust invariant representation learning.


==> Bispectral Neural Networks ICLR Camera Ready/sections/1-introduction.tex <==
\section{Introduction}

\vspace{-0.2cm}
A fundamental problem of intelligence is to model the transformation structure of the natural world.  In the context of vision, translation, rotation, and scaling define symmetries of object categorization\textemdash the transformations that leave perceived object identity invariant. In audition, pitch and timbre define symmetries of speech recognition. Biological neural systems have learned these symmetries from the statistics of the natural world\textemdash either through evolution or accumulated experience. Here, we tackle the problem of learning symmetries in artificial neural networks. 

At the heart of the challenge lie two requirements that are frequently in tension: \textit{invariance} to transformation structure and \textit{selectivity} to pattern structure. In deep networks, operations such as \texttt{max} or \texttt{average} are commonly employed to achieve invariance to local transformations. Such operations are invariant to many natural transformations; however, they are also invariant to unnatural transformations that destroy image structure, such as pixel permutations. This lack of selectivity may contribute to failure modes such as susceptibility to adversarial perturbations \cite{goodfellow2014explaining}, excessive invariance \cite{jacobsen2018excessive}, and selectivity for textures rather than objects \cite{brendel2019approximating}. Thus, there is a need for computational primitives that selectively parameterize natural transformations and facilitate robust invariant representation learning.

An ideal invariant would be \textit{complete}. A complete invariant preserves all pattern information and is invariant only to specific transformations relevant to a task. Transformations in many datasets arise from the geometric structure of the natural world. The mathematics of \textit{groups} and their associated objects give us the machinery to precisely define, represent, and parameterize these transformations, and hence the problem of invariant representation learning. In this work, we present a novel neural network primitive based on the \textit{bispectrum}, a complete invariant map rooted in harmonic analysis and group representation theory \cite{kakarala1993group}. 

Bispectral Neural Networks flexibly parameterize the bispectrum for arbitrary compact commutative groups, enabling both the group and the invariant map to be learned from data. The architecture is remarkably simple. It is comprised of two layers: a single learnable linear layer, followed by a fixed collection of triple products computed from the output of the previous layer. BNNs are trained with an objective function consisting of two terms: one that collapses all transformations of a pattern to a single point in the output (invariance), and another that prevents information collapse in the first layer (selectivity). 

 We demonstrate that BNNs trained to separate orbit classes in augmented data learn the group its Fourier transform, and corresponding bispectrum purely from the symmetries implicit in the data (Section \ref{section:learningirreps}). Because the model has learned the fundamental structure of the group, we show that it generalizes to novel, out-of-distribution classes with the same group structure and facilitates downstream group-invariant classification (Section \ref{section:classification}). Further, we demonstrate that the trained network inherits the completeness of the analytical model, which endows the network with strong adversarial robustness (Section \ref{section:adversarial}). Finally, we demonstrate that the weights of the network can be used to recover the group Cayley table\textemdash the fundamental signature of a group's structure (Section \ref{section:cayley}). Thus, an explicit model of the group can be learned and extracted from the network weights. To our knowledge, our work is the first to demonstrate that either a bispectrum or a group Cayley table can be learned from data alone. Our results set the foundation of a new computational primitive for robust and interpretable representation learning.

\vspace{-0.25cm}
\subsection{Related Work}
\vspace{-0.25cm}

The great success and efficiency of convolutional neural networks owe much to built-in \textit{equivariance} to the group of 2D translations. In recent years, an interest in generalizing convolution to non-Euclidean domains such as graphs and 3D surfaces has led to the incorporation of additional group symmetries into deep learning architectures \cite{cohen2016group, bronstein2021geometric}. In another line of work, Kakarala \cite{kakarala2012bispectrum} and Kondor \cite{kondor2007novel} pioneered the use of the analytical group-invariant bispectrum in signal processing and machine learning contexts. Both of these approaches require specifying the group of transformations \textit{a priori} and explicitly building its structure into the network architecture.  
However, the groups that structure natural data are often either unknown or too complex to specify analytically\textemdash for example, when the structure arises from the interaction of many groups, or when the group acts on latent features in data. 

Rather than building in groups by hand, another line of work has sought to \textit{learn} underlying group structure solely from symmetries contained in data. The majority of these approaches use structured models that parameterize irreducible representations or Lie algebra generators, which act on the data through the group exponential map \cite{rao1999learning,miao2007learning,culpepper2009learning,sohl2010unsupervised,cohen2014learning,chau2020disentangling}. In these models, the objective is typically to infer the group element that acts on a template to generate the observed data, with inference accomplished through Expectation Maximization or other Bayesian approaches. A drawback of these models is that both the exponential map and inference schemes are computationally expensive. Thus, they are difficult to integrate into large-scale systems. A recent feed-forward approach \cite{benton2020learning} learns distributions over the group of 2D affine transformations in a deep learning architecture. However, the group is not learned in entirety, as it is restricted to a distribution on a pre-specified group.

Here, we present a novel approach for learning groups from data in an efficient, interpretable, and fully feed-forward model that requires no prior knowledge of the group, computation of the exponential map, or Bayesian inference. The key insight in our approach is to harness the generality of the form of the group-invariant bispectrum, which can be defined for arbitrary compact groups. Here, we focus on the class of compact commutative groups.

\vspace{-0.15cm}


==> Bispectral Neural Networks ICLR Camera Ready/sections/2-bispectrum.tex <==
\section{The Bispectrum}\label{section:bispectrum}

\vspace{-0.25cm}


The theory of groups and their representations provides a natural framework for
constructing computational primitives for robust machine learning systems. We provide a one-page introduction to these mathematical foundations in Appendix \ref{appendix:math}. Extensive treatment of these concepts can be found in the textbooks of Hall \cite{hall2013lie} and Gallier \& Quaintance \cite{gallier2020differential}. We now define the concepts essential to this work: invariance, equivariance, orbits, complete invariance, and irreducible representations.

Let $G$ be a group, $X$ a space on which $G$ acts, and $f$ a signal defined on the domain $X$. The \textit{orbit} of a signal is the set generated by acting on the domain of the signal with each group element, i.e. $\{f(gx) : g \in G \}$. In the context of image transformations this is the set of all transformed versions of a canonical image\textemdash for example, if $G$ is the group $SO(2)$ of 2D rotations, then the orbit contains all rotated versions of that image. 

A function $\phi: X \to Y$ is $G$-\textit{equivariant} if $\phi(g x) = g^\prime \phi(x)$ for all $g \in G$ and $x \in X$, with $g^\prime \in G^\prime$ homomorphic to $G$. That is, a group transformation on the input space results in a corresponding group transformation on the output space. A function $\phi: X \to Y$ is $G$-\textit{invariant} if $\phi(x) = \phi(g x)$ for all $g \in G$ and $x \in X$. This means that a group action on the input space has no effect on the output. We say $\phi$ is a \textit{complete invariant} when $\phi(x_1) = \phi(x_2)$ if and only if $x_2 = g x_1$ for some $g \in G$ and $x_1,x_2 \in X$. A complete invariant collapses each orbit to a single point while also guaranteeing that different orbits map to different points. In the context of rotation-invariant vision, for example, this would mean that the only information lost through the map $\phi$ is that of the specific ``pose'' of the object.

A \textit{representation} of a group G is a map $\rho: G \rightarrow GL(V)$ that assigns elements of $G$ to elements of the group of linear transformations (e.g. matrices) over a vector space $V$ such that $\rho(g_1 g_2) = \rho(g_1) \rho(g_2)$. That is, $\rho$ is a group homomorphism. In our case, $V$ is $\mathbb{C}^n$. A representation is \textit{reducible} if there exists a change of basis that decomposes the representation into a direct sum of other representations. An \textit{irreducible representation} is one that cannot be further reduced in this manner, and the set $Irr(G)$ are often simply called the \textit{irreps} of $G$. The irreducible representations of all finite commutative groups are one-dimensional (therefore equivalent to the characters of the irreps), and in bijection with the group itself. 

\vspace{-0.25cm}

\subsection{Fourier Analysis on Groups}
\vspace{-0.25cm}

A powerful approach for constructing invariants leverages the group theoretic generalization of the classical Fourier Transform \cite{rudin1962fourier}. Let $f(g): G \rightarrow \mathbb{R}$ be a signal on a group $G$, and let $Irr(G)$ denote the irreducible representations of the group. We assume that $\rho \in Irr(G)$ are also \textit{unitary} representations (i.e., $\rho^{-1} = \rho^{\dagger}$, with $\rho^{\dagger}$ the conjugate transpose). The \textit{Generalized Fourier Transform} (GFT) is the linear map $f \mapsto \hat{f}$, in which Fourier frequencies are indexed by $\rho \in Irr(G)$:
\begin{equation}
\hat{f}_{\rho} = \sum_{g \in G} \rho(g)f(g).
\end{equation} 
 Readers familiar with the classical Fourier transform should identify $\rho(g)$ with the exponential term in the usual sum or integral.  Here, they arise naturally as the representations of $\mathbb Z/n \mathbb Z$ or $S^1$. Intuitively, these $\rho$ are the ``fundamental frequencies" of the group. In particular, for $G = \mathbb Z/n \mathbb Z$\textemdash the group of \textit{integers modulo $n$}\textemdash they are the classical $n$ discrete Fourier frequencies: $\rho_k(g) = e^{-\mathbf{i} 2 \pi  k g / n}$, for $k=0,\ldots,n-1$ and $g \in \mathbb Z/n \mathbb Z$. For compact continuous groups $G$, the sum above is replaced by an integral $\int \rho(u)f(u) du$ over a Haar measure $du$ for the group.
 
 Importantly, the Fourier transform is \textit{equivariant} to the action of translation on the domain of the input\textemdash a fundamental, if not defining, property. That is, if $f^t = f(g-t)$ is the translation of $f$ by $t \in G$, its Fourier transform becomes: 
\begin{equation}
(\hat{f^t})_{\rho} = \rho(t) \hat{f}.
\end{equation} 
For the classical Fourier transform, this is the familiar \textit{Fourier shift property}: translation of the input results in phase rotations of the complex Fourier coefficients. This property is exploited in one well-known Fourier invariant\textemdash the \textit{power spectrum}:
\begin{equation}
    q_{\rho} = \hat{f}^{\dagger}_{\rho} \hat{f}_{\rho}.
\end{equation}

The power spectrum preserves only the magnitude of the Fourier coefficients, eliminating the phase information entirely by multiplying each coefficient by its conjugate:
\begin{eqnarray*}
  q^t_k = \Big(e^{-\mathbf{i}2\pi k t / n}  \hat{f}_k\Big)^{\dagger} \Big(e^{-\mathbf{i}2\pi k t / n} \hat{f}_k\Big) =  e^{\mathbf{i}2\pi k t / n} e^{-\mathbf{i}2\pi k t / n}  \hat{f}_k^{\dagger} \hat{f}_k  = q_k.
\end{eqnarray*}
Although this approach eliminates variations due to translations of the input, it also eliminates much of the signal structure, which is largely contained in relative phase relationships \cite{oppenheim1981importance}. Thus, the power spectrum is \textit{incomplete}.  As a result, 
it is easy to create ``adversarial examples'' demonstrating the incompleteness of this invariant: any two images with identical Fourier magnitudes but non-identical phase have the same power spectra (Appendices \ref{appendix:powerspectrum} and \ref{appendix:completeness}).

\vspace{-0.25cm}
\subsection{The Bispectrum}
\vspace{-0.25cm}

The \textit{bispectrum} is a lesser known Fourier invariant parameterized by pairs of frequencies in the Fourier domain. The translation-invariant \textit{bispectrum} for 1D signals $f \in \mathbb R^n$ is the complex matrix $B \in \mathbb C^{n \times n}$:
\begin{equation}
B_{i,j} = \hat{f}_i \hat{f}_j \hat{f}_{i+j}^{\dagger},
\end{equation}
where $\hat{f} = (\hat{f}_0,\ldots,\hat{f}_{n-1})$ is the 1D Fourier transform of $f$ and the sum $i+j$ is taken modulo $n$.  Intuitively, bispectral coefficients $B_{ij}$ indicate the strength of couplings between different phase components in the data, preserving the phase structure that the power spectrum loses. Again, the equivariance property of the GFT is key to $B$'s invariance. Like the power spectrum, it cancels out phase shifts due to translation. However it does so while preserving the relative phase structure of the signal.  This remarkable property may be seen as follows:

\begin{eqnarray*}
B^t_{k_1, k_2} &=& e^{-i 2 \pi k_1 t / n} \hat{f}_{k_1}  e^{-\mathbf{i} 2 \pi k_2 t/ n} \hat{f}_{k_2} e^{\mathbf{i} 2 \pi (k_1+k_2) t / n} \hat{f}^{\dagger}_{k_1 + k_2} \\
 &=& e^{-\mathbf{i} 2 \pi k_1 t / n} e^{-\mathbf{i} 2 \pi k_2 t/ n} e^{\mathbf{i} 2 \pi k_1 t / n} e^{\mathbf{i} 2 \pi k_2 t / n}\hat{f}_{k_1} \hat{f}_{k_2} \hat{f}^{\dagger}_{k_1 + k_2} = B_{k_1, k_2}.
 \label{eq:bispectrum}
\end{eqnarray*}


 Unlike the power spectrum, the bispectrum (for compact groups) is complete and can be used to reconstruct the original signal up to translation \cite{yellott1992uniqueness}. More generally, the bispectrum is defined for arbitary compact groups:

\begin{equation}
B_{\rho_i, \rho_j} = \hat{f}_{\rho_i}\hat{f}_{\rho_j}\hat{f}_{\rho_i \rho_j}^{\dagger},
\end{equation}
 
 with the addition modulo $n$ replaced by the group product.  For non-commutative groups, the bispectrum has a similar structure, but is modified to accommodate the fact that the irreps of non-commutative groups map to matrices rather than scalars (Appendix \ref{appendix:_non-commutative-bispectrum}).

Historically, the bispectrum emerged from the study of the higher-order statistics of non-Gaussian random processes, and was used as a tool to measure the non-Gaussianity of a signal \cite{tukey1953spectral, brillinger1991some, nikias1993signal}. The work of Yellott and Iverson \cite{yellott1992uniqueness} established that every integrable function with compact support is completely identified\textemdash up to translation\textemdash by its three-point autocorrelation and thus its bispectrum (Appendix \ref{appendix:autocorrelation}). Later work of Kakarala tied the bispectrum to the more general formulation of Fourier analysis and thus defined it for all compact groups \cite{kakarala1993group, kakarala2012bispectrum}. Kakarala went on to prove that it is complete \cite{kakarala2009completeness} in both commutative and non-commutative formulations (Appendix \ref{appendix:completeness}).


==> Bispectral Neural Networks ICLR Camera Ready/sections/3-bispectral-networks.tex <==
\vspace{-0.15cm}
\section{Bispectral Neural Networks}
\vspace{-0.25cm}

\label{section:bnns}
We draw inspiration from the group-invariant bispectrum to define Bispectral Neural Networks, a neural network architecture that parameterizes the \textit{ansatz} of the bispectrum. The key idea behind this approach is to constrain the optimization problem by building in the \textit{functional form} of a solution known to exist. Importantly, we build in only the generic functional form and allow the network to learn the appropriate parameters (and thus the group over which it is defined) from data. We draw upon two key properties of the bispectrum, which allow it to be naturally parameterized and learned:

\begin{enumerate}[leftmargin=*]
    \item The bispectrum is computed on a group-equivariant Fourier transform. The Fourier transform is a linear map and can be written as $z = Wx$, with $W$ a matrix of irreducible representations\textemdash the Discrete Fourier Transform (DFT) matrix, in the classical case. If the group is unknown, we can treat $W$ as a matrix of parameters to be learned through optimization. The bispectrum computation is identical regardless of the structure of the irreps; thus we can use a single network architecture to learn finite approximations of arbitrary compact commutative groups.
    \item The bispectrum separates orbits. Here, we use orbit separation at the output of the bispectrum computation as the criterion to optimize the parameters defining the group-equivariant Fourier transform. This requires knowing only which datapoints are in the same orbit (but not the group that generates the orbit), and is similar in spirit to contrastive learning \cite{hadsell2006dimensionality}. 
\end{enumerate}

\vspace{-0.25cm}
\subsection{Model Architecture}
\label{section:architecture}
\vspace{-0.25cm}

Concretely, given an input vector $x \in \mathbb{R}^n$, the Bispectral Neural Network module is completely specified by one complex matrix $W \in \mathbb{C}^{n \times n}$, where each row $W_i \in \mathbb{C}^{n}$ plays the role of an irreducible representation. This matrix defines the linear transformation:
\begin{equation}
    z = Wx.
    \label{eq:linear-map}
\end{equation}
If $W$ defines a Fourier transform on $G$, then each element of $z$ is a coefficient on a different irreducible representation of $G$. The analytical bispectrum can then be computed from triples of coefficients as:
\begin{equation}
    B_{i, j} = z_i z_j z_{ij}^{\dagger}
    \label{eq:bispectrum_z}
\end{equation}
However, if the group is unknown, then 
we do not know the product structure of the group and thus do not know \textit{a priori} which element in the vector $z$ corresponds to the $(ij)$\textsuperscript{th} irrep. Conveniently, for commutative groups, all irreducible representations are in bijection with the group elements. That is, each irreducible representation can be uniquely identified with a group element. Consequently, the $(ij)$\textsuperscript{th} representation can obtained from the element-wise multiplication of the $i$\textsuperscript{th} and $j$\textsuperscript{th} irreducible representations. Thus, the (conjugated) $(ij)$\textsuperscript{th} coefficient can be obtained as
\begin{equation}
    z_{ij}^{\dagger}= (W_i \odot W_j)^{\dagger}x,
\end{equation}
with $\odot$ indicating the Hadamard (element-wise) product and $^\dagger$ the complex conjugate. Plugging this into Equation \ref{eq:bispectrum_z} and expanding the terms, we obtain the Bispectral Network:
\begin{equation}
    \beta_{i,j} (x) = W_i x \cdot  W_j x \cdot (W_i \odot W_j)^\dagger x
    \label{eq:bs-net}
\end{equation}

Figure \ref{fig:model-schematic} illustrates the computation. Each linear term $W_i x$ is an inner product yielding a scalar value, and the three terms are combined with scalar multiplication in $\mathbb{C}$.   Note that this equation shows the computation of a single scalar output $\beta_{i,j}$. In practice, this is computed for all non-redundant pairs.

\begin{figure}[H]
\vspace{-0.25cm}
    \centering
    \includegraphics[width=\linewidth]{figs/bnns-schematic.png}
    \caption{\textbf{Bispectral Neural Networks}. A single linear neural network layer parameterized by $W$ generates the output $z = Wx$. Pairs of coefficients $z_i$ and $z_j$ and the corresponding weights $W_i$ and $W_j$ are then used to compute the output of the network $\beta_{i,j} = z_i z_j z_{ij}^\dagger$, with $z_{ij}$ computed as $(W_i \odot W_j)x$. Here, the weights are depicted as the canonical Fourier basis on $\mathbb{S}^1$ for illustrative purposes. In practice, the weights are randomly initialized, but are expected to converge to the irreps of the group that structures the dataset. \vspace{-0.5cm}}
    \label{fig:model-schematic}
\end{figure}

While the bispectrum is a third-order polynomial, it results in only $n^2$ rather than $n^3$ products, due to the constraint on the third term. Moreover, the bispectrum has many symmetries and is thus highly redundant. The most obvious symmetry is reflection over the diagonal\textemdash i.e. $\beta_{i, j} = \beta_{j, i}$. However, there are many more (see Appendix \ref{appendix:symmetries}). Here, we compute only the upper triangular of the matrix.

As the Bispectral Network computes third-order products of the input, the output values can be both very large and very small, which can result in numerical instability during optimization. To combat this, we normalize the output of the network to the unit sphere in $\mathbb{C}^n$:
\begin{equation}
    \bar{\beta}(x) = \frac{\beta(x)}{||\beta(x)||_2}
    \label{eq:normed-bs-net}
\end{equation}
We demonstrate in Appendix \ref{appendix:_normalized_completeness} that the analytical bispectrum can be normalized to the unit sphere while preserving completeness up to a scalar factor (Appendix \ref{appendix:_normalized_completeness}, Theorem \ref{norm_bispectrum_thm}). Thus, we similarly expect that this normalization will not impact the robustness of the network.

\vspace{-0.25cm}
\subsection{Orbit Separation Loss}
\vspace{-0.25cm}

Given a dataset $X = \{x_1, ..., x_m\}$ with latent group structure and labels $Y = \{y_1, ..., y_m\}$ indicating which datapoints are equivalent up to transformation (but without information about the transformation itself, i.e. \textit{how} they are related), we wish to learn an invariant map that collapses elements of the same group orbit and separates distinct orbits. Critically, we want this map to be both \textit{invariant} to group actions and \textit{selective} to pattern structure\textemdash that is, to be \textit{complete} \cite{kakarala2009completeness}. A network that successfully learns such a map will have implicitly \textit{learned the group} that structures transformations in the data. 

To that end, we introduce the \textit{Orbit Separation Loss}. This loss encourages the network to map elements of the same orbit to the same point in the representation space, while ensuring degenerate solutions (i.e. mapping all inputs to the same point) are avoided:
\begin{equation}
    L(x_a) = \sum_{j | y_b = y_a}||\bar{\beta}(x_a) - \bar{\beta}(x_b)||_2^2 + \gamma ||x_a - W^{\dagger}W\,x_a||_2^2.
\label{eq:loss-function1}
\end{equation}
 The first term measures the Euclidean distance in the output space between points in the same orbit. Thus, minimizing the loss encourages them to be closer. In the second term, the input $x_a$ is reconstructed by inverting the linear transform as $W^{\dagger}Wx_a$. The second term is thus a measure of whether information is preserved in the map. During training, each row vector in the weight matrix $W$ is normalized to unit length after every gradient update, which pushes $W$ towards the manifold of unitary matrices. The coefficient $\gamma$ weights the contribution of the reconstruction error to the loss.





==> Bispectral Neural Networks ICLR Camera Ready/sections/4-results.tex <==

\vspace{-0.25cm}
\section{Experiments and Analyses}
\vspace{-0.25cm}

We now test the capacity of Bispectral Networks to learn a group by learning to separate orbit classes.  We conduct four experiments to analyze the properties of the architecture: learning Fourier transforms on groups (Section \ref{section:learningirreps}), group-invariant classification (Section \ref{section:classification}), model completeness (Section \ref{section:adversarial}), and extracting the Cayley table (Section \ref{section:cayley}).

\vspace{-0.25cm}
\subsection{Learning Fourier Transforms on Groups}
\label{section:learningirreps}
\vspace{-0.25cm}



We first examine whether Bispectral Networks trained to separate orbit classes will learn the Fourier transform and corresponding bispectrum of the group that structures the data. Here, we test the network on two groups, which act on the image grid to generate image orbits. The first is one whose bispectrum is known and well-understood: the group $\mathbb{S}^1 \times \mathbb{S}^1$ of 2D cyclic translations, i.e. the canonical 2D Fourier transform. The second is the group $SO(2)$. To our knowledge, a bispectrum on $SO(2)$ acting on the grid (or disk) has not been defined in the mathematics literature, as the domain is not a homogeneous space for the group\textemdash an assumption fundamental to much of bispectrum theory. However, a Fourier transform for $SO(2)$ acting on the disk has been defined \cite{verrall1998disk} using the orthogonal basis of disk harmonics. We thus expect our weight matrix $W$ to converge to the canonical Fourier basis for the group $\mathbb{S}^1 \times \mathbb{S}^1$, and hypothesize the emergence of disk harmonics for $SO(2)$.

Models are trained on datasets consisting of 100 randomly sampled (16, 16) natural image patches from the van Hateren dataset \cite{van1998independent} that have been transformed by the two groups to generate orbit classes. Further details about the dataset can be found in Appendix \ref{appendix:_dataset}. Networks are trained to convergence on the Orbit Separation Loss, Equation \ref{eq:loss-function1}. All hyperparameters and other details about the training procedure can be found in Appendix \ref{appendix:training}.1. 

Remarkably, we find that the relatively loose constraints of the orbit separation loss and the product structure of the architecture is sufficient to encourage the network to learn a group-equivariant Fourier transform and its corresponding bispectrum from these small datasets. This is observed in the structure of the network weights, which converge to the irreducible representations of the group in the case of $\mathbb{S}^1 \times \mathbb{S}^1$, and filters resembling the disk harmonics for $SO(2)$) (Figure \ref{fig:translation-weights}). Importantly, we observe that the learned linear map (Equation \ref{eq:linear-map}) is equivariant to the action of the group on the input, and the output of the network (Equation \ref{eq:normed-bs-net}) is invariant to the group action on arbitrary input signals. We visualize this in Figure \ref{fig:translation-inv-eq} for transformed exemplars from the MNIST dataset, which the model was not trained on, demonstrating the capacity of the model to generalize these properties to out-of-distribution data.

\vspace{-0.2cm}
\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{figs/learned-filters.png}
    \caption{\textbf{Filters Learned in Bispectral Networks}. Real components of weights learned in the Bispectral Network trained on the transformed van Hateren Natural Images datasets, for $\mathbb{S}^1 \times \mathbb{S}^1$ 2D Translation (left) and $SO(2)$ 2D Rotation dataset (right). The full set of learned weights can be found in Appendix \ref{appendix:irreps}. \vspace{-0.3cm}}
    \label{fig:translation-weights}
\end{figure}

 \begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figs/inv-eq.png}
    \caption{\textbf{Model Outputs on Transformed Data.} Real components of the outputs of the linear transform ($Wx$, top row) and full network output (Eq. \ref{eq:normed-bs-net}, bottom row). Data inputs are cyclically translated/rotated in one direction (x-axis) and layer/network outputs are computed for each transformation. Each colored line represents the output of a single neuron, with the activation value on the y-axis. In the top row, only four neuron outputs are visualized, for clarity. The equivariance of the first layer is observed in the sinuisoidal responses, which reveal equivariant phase shifts on each neuron's output as the input transforms. The invariance of the network output is observed in the constant response across all translated or rotated images.\vspace{-0.5cm}}
    \label{fig:translation-inv-eq}
\end{figure}

\subsection{Group-Invariant Classification}
\label{section:classification}


  We next examine the utility of the rotation model learned in Section \ref{section:learningirreps} for facilitating performance on a downstream image classification task: digit classification for the Rotated MNIST dataset. For this experiment, we append a simple multi-layer fully-connected ReLU network (MLP; the ``classification network'') to the output of the Bispectral Network and train it on the classification objective. While the Bispectral Network learns to eliminate factors of variation due to group actions, the classification network learns to eliminate other variations within digit classes irrelevant to classification, i.e. those due to handwriting style.  We train the classification model using the scheme described in Appendix \ref{appendix:training}. We compare the performance of our model to four leading approaches to group-invariant classification, in addition to a Linear Support Vector Machine (SVM) model that we train as a baseline (Table \ref{table:classification}). 
 
Our model obtains a competitive 98.1\% classification accuracy on this task\textemdash within $0.2$ - $1.2\%$ of the state-of-the-art methods compared to here. It also possesses several notable differences and advantages to the models presented in this table. First, our model \textit{learns the group} from data, in contrast to Harmonic Networks and E2CNNs\textemdash which build in $SO(2)$-equivariance\textemdash and Augerino, which learns a distribution over the pre-specified group of 2D affine transformations. Although our method is marginally outperformed by these models in terms of classification accuracy, ours outperforms \cite{cohen2014learning}, the only other model that fully learns a group. Second, our model is fully feed-forward, and it does not rely on the computationally intensive EM inference scheme used in \cite{cohen2014learning}, or the exponential map as used in \cite{cohen2014learning} and \cite{benton2020learning}. Finally, in the next section, we demonstrate that our model is approximately \textit{complete}. By contrast, we demonstrate, representations within the leading models E2CNN and Augerino exhibit excessive invariance. 

 
\begin{table}[H]
    \centering
        \vspace{-0.35cm}
        \footnotesize
            \begin{tabular}{lcccc}\\ \toprule  
            \textbf{Model} & \textbf{Learns} & \textbf{Fully} & \textbf{Approximately} & \textbf{RotMNIST}\\
             & \textbf{Group} & \textbf{Feedforward} & \textbf{Complete} & \textbf{Accuracy} \\
            \midrule
            Linear SVM (Baseline) & N & NA & - & 54.7\% \\ 
            \midrule
            Cohen \& Welling (2014) \cite{cohen2014learning} & \textbf{Y} & N & - & $\sim$ 97\%$^\dagger$\\  
            \midrule
            Harmonic Networks (2017) \cite{worrall2017harmonic}& N & \textbf{Y} & - & 98.3\% \\ 
            \midrule
            Augerino (2020) \cite{benton2020learning} & \textbf{Y}$^*$  & \textbf{Y} & N &  98.9\%\\  
            \midrule
            E2CNN (2019) \cite{weiler2019general} & N & \textbf{Y} & N & \textbf{99.3}\% \\  
            \midrule
            \textbf{Bispectral Network + MLP} & \textbf{Y} & \textbf{Y} & \textbf{Y} & 98.1\% \\  
            \bottomrule
            \end{tabular}
    
    \caption{\label{table:classification} \textbf{Model Comparison on RotMNIST}. \footnotesize  Bispectral Networks achieve 98.1\% classification accuracy on RotMNIST. The model is marginally outperformed by three models that require the partial or complete specification of the group structure in their design. Our model, by contrast \textit{learns} the group entirely from data. Further, our model is approximately complete, while the leading models E2CNN and Augerino exhibit excessive invariance (Figure \ref{fig:adversarial-examples}). 
    \vspace{0.1cm}
    \\ \scriptsize $^\dagger$This number was estimated from the bar plot in Figure 4 of  \cite{cohen2014learning} and approved  by the first author of the paper in personal communication.\vspace{-0.03cm}
    \\ $^*$ The model in \cite{benton2020learning} learns a \textit{distribution} over a pre-specified group. It is different in kind to \cite{cohen2014learning} and our model, which learn the group itself.
    \vspace{-0.4cm} }
\end{table}

\vspace{-0.3cm}

\subsection{Model Completeness}
\label{section:adversarial}

A key property of the analytical bispectrum is its \textit{completeness}: only signals that are exactly equal up to the group action will map to the same point in bispectrum space. Here, we analyze the completeness of the trained models, using \textit{Invariance-based Adversarial Attacks} (IAAs) \cite{jacobsen2018excessive} as a proxy. IAAs aim to identify  \textit{model metamers}\textemdash inputs that yield identical outputs in the model's representation space, but are perceptually dissimilar in the input space. For an approximately complete model, we expect all inputs that map to the same point in model representation space to belong to the same orbit. That is, the only perturbations in pixel space that will give rise to identical model representations are those due to the group action.

We test the completeness of the trained models as follows. A batch of targets $\{x_1, ..., x_N\}$, $x \in \mathbb{R}^m$ are randomly drawn from the RotMNIST dataset. A batch of inputs $\{ \bar{x}_1, ..., \bar{x}_N \}$ , $\bar{x} \in \mathbb{R}^m$ are randomly initialized, with pixels drawn from a standard normal distribution. Both the targets and random inputs are passed through the network to yield $\bar{\beta}(x_i)$ (target) and $\bar{\beta}(\bar{x}_i)$ (adversary). The following objective is minimized with respect to the $\bar{x}_i$:
\begin{equation}
    L = \sum_{i=0}^{N}||\bar{\beta}(x_i) - \bar{\beta}(\bar{x}_i)||_2^2
\label{eq:loss-function}
\end{equation}

An optimized input $\bar{x}_i$ is considered a model metamer if it yields a model representation within $\epsilon$ of $\bar{\beta}(x_i)$, is classified equivalently as $x_i$, but is not in the orbit of $x_i$. Here, we aim to minimize distance between targets and adversaries in the \textit{model representation space}\textemdash i.e. the output of the Bispectral Network, prior to the classification model. For the comparison models E2CNN and Augerino, we use the output of the layer prior to the softmax.

Figure \ref{fig:adversarial-examples} shows the targets and the optimized adversarial inputs for the Bispectral Network trained on rotation in the van Hateren dataset, and the E2CNN and Augerino models trained on Rotated MNIST. For the Bispectral Network, we observe that all random initializations consistently converge to an element within the orbit of the target, indicating that the invariant map learned by the model is close to complete.  By contrast, many unrelated or noisy metameric images can be found for E2CNN and Augerino. These metamers yield identical model representations (up to $\epsilon$) and identical classifications as the targets, but are not contained in their orbits of the targets. Interestingly, the metamers optimized for Augerino possess structure that at times resembles features in the target image. We roughly estimate the percentage of these ``perceptually similar'' inputs as $35\%$. The model nonetheless exhibits excessive invariance and is not complete. 

    \vspace{-0.4cm}


\begin{figure}[H]
    \centering
    \includegraphics[trim={0 0 0 0cm},clip, width=\linewidth]{figs/completeness.png}
    \caption{\textbf{Completeness in Bispectral Networks.} Targets and optimized inputs for (left) E2CNN, (middle) Augerino, and (right) Bispectral Networks. Images are randomly initialized and optimized to yield representations identical to a target image. If a model possesses excessive invariance, there exist images that will yield equivalent representations while being non-equivalent up to the group action.  For Bispectral Networks, all optimized inputs are within the orbits of the targets, indicating approximate completenes. By contrast, many model metamers are found for E2CNN and Augerino. \vspace{-0.4cm}
}
    \label{fig:adversarial-examples}
\end{figure}

\vspace{-0.5cm}

\subsection{Learning the Group: Extracting the Cayley Table}
\label{section:cayley}
\vspace{-0.25cm}


 Finally, we demonstrate that the converged network weights can be used to \textit{construct the group itself}\textemdash i.e. the product structure of the group, as captured by the group's Cayley table. For finite groups, a Cayley table provides a complete specification of group structure. Here, we demonstrate a novel method for constructing a Cayley table from learned irreps, described in in Appendix \ref{appendix:cayley}, which exploits the bijection between irreps and group elements in commutative groups.

We test this approach on all unique finite commutative groups of order eight: $\mathbb{Z}/8\mathbb{Z}$, $\mathbb{Z}/4\mathbb{Z} \times \mathbb{Z}/2\mathbb{Z}$, and $\mathbb{Z}/2\mathbb{Z} \times \mathbb{Z}/2\mathbb{Z} \times \mathbb{Z}/2\mathbb{Z}$. For each group, we generate a synthetic dataset consisting of 100 random functions over the group, $f: G \to \mathbb{R}$, with values in $\mathbb{R}$ drawn from a standard normal distribution, and generate the orbit of each exemplar under the group. Networks are trained to convergence on each dataset using the Orbit Separation Loss, Equation \ref{eq:loss-function1}. Details about the training procedure can be found in Appendix \ref{appendix:cayley-training}. After a model has converged, we use its learned weights to compute a Cayley table using Algorithm \ref{alg:cayley_from_irreps} in Appendix \ref{appendix:cayley}. We check the isomorphism of the learned Cayley table with the ground truth using Algorithm \ref{alg:isIsomorphic} in Appendix \ref{appendix:cayley}.

\vspace{-0.1cm}

\vspace{-0.2cm}
\begin{figure}[H]
    \centering
    \includegraphics[width=\linewidth]{figs/cayley-tables.png}
    \caption{\textbf{Learned Cayley Tables for All Unique Groups of Order Eight}. Rows and columns are labeled with integers that index group elements. Each cell of the table contains the index of the group element obtained by composing the group elements indexed in the row and column. The Cayley table thus contains all information about the group structure. Bispectral Networks perfectly recover the Cayley tables for all groups tested here. \vspace{-0.5cm}}
    \label{fig:learned-cayley}
\end{figure}


Strikingly, we are able to recover the exact structure of the groups that generated the data orbits from the converged models' weights, in the form of the Cayley tables displayed in Figure \ref{fig:learned-cayley}. For each dataset, the recovered Cayley tables are identical to the known ground-truth Cayley tables. To our knowledge, this is the first demonstration that an explicit representation of the product structure of an unknown group can be learned from data. Our results on all finite commutative groups of order eight suggest that this will generalize more broadly to all finite commutative groups.



==> Bispectral Neural Networks ICLR Camera Ready/sections/5-discussion.tex <==

\vspace{-0.3cm}
\section{Discussion}

\vspace{-0.3cm}

In this work, we introduced a novel method for learning groups from data in a neural network architecture that simultaneously learns a group-equivariant Fourier transform and its corresponding group-invariant bispectrum. The result is an interpretable model that learns the irreducible representations of the group, which allow us to recover an explicit model of the product structure of the group\textemdash i.e. the group itself, in the form of its Cayley table. The resulting trained models are both powerful and robust\textemdash capable of generalizing to arbitrary unseen datasets that are structured by the same transformation group, while exhibiting approximate \textit{completeness}. To our knowledge, these results provide the first demonstration that a bispectrum or Cayley table can be learned simply from the symmetries in data alone. We view the work presented here as a starting point for learning the more complex groups needed to recognize 3D objects in natural imagery. In ongoing work, we are extending the model to the non-commutative form of the bispectrum (Appendix \ref{appendix:_non-commutative-bispectrum}), and developing a localized version amenable to stacking hierarchically in deep networks.

The precise convergence of the Bispectral Network parameters to canonical forms from representation theory\textemdash under the relatively weak constraints of the third-order model ansatz and the orbit separation loss\textemdash suggests the uniqueness of this solution within the model class. Indeed, the Fourier solution is likely guaranteed by the uniqueness of the bispectrum as a third-order polynomial invariant \cite{sturmfels2008algorithms}. Future work should explore the bounds of these guarantees in the context of statistical learning. We venture to suggest further that the uniqueness and completeness of the bispectrum make it a compelling candidate computational primitive for invariant perception in artificial and biological systems alike. Indeed, results from across areas of visual cortex suggest that group representations may play an important role in the formation of visual representations in the brain \cite{sanborn-thesis}. Models like the one presented here may provide concrete hypotheses to test in future mathematically motivated neuroscience research. 


\newpage 

